Nurturing Lyman Break Galaxies: Observed link between environment and spectroscopic features

We examine the effects of magnitude, colour, and Ly-alpha equivalent width (EW) on the spatial distribution of z~3 Lyman break galaxies (LBGs) and report significant differences in their auto-correlation functions (ACFs). The results are obtained using samples of ~10,000-57,000 LBGs from the Canada-France-Hawaii Telescope Legacy Survey. We find that magnitude has a larger effect on the ACF amplitude on small scales (<~1 Mpc) and that colour is more influential on large scales (>~1 Mpc). We find the most significant differences between ACFs for LBGs with dominant net Ly-alpha EW in absorption (aLBGs) and dominant net Ly-alpha EW in emission (eLBGs) determined from >~95% pure samples of each population using a photometric technique calibrated from ~1000 spectra. The aLBG ACF one-halo term departs from a power law fit near ~1 Mpc, corresponding to the virial radii of M_DM ~10^13 M_solar haloes, and shows a strong two-halo term amplitude. In contrast, the eLBG ACF one-halo term departs at ~0.12 Mpc, suggesting parent haloes of M_DM ~10^11 M_solar, and a two-halo term that exhibits a `hump' on intermediate scales that we localize to the faintest, bluest members. We find that the `hump' can be well fit with a model in which a significant fraction of eLBGs reside on shells. The auto- and cross-correlation functions indicate that aLBGs are found in massive, group-like haloes and that eLBGs are found largely on group outskirts and in the field. Ly-alpha is a tracer of several intrinsic LBG properties, including morphology, implying that the mechanisms behind the morphology-density relation are in place at z~3 and that Ly-alpha EW may be a key environment diagnostic. Finally, our results show that the mass of LBGs has been underestimated because the LBG ACF amplitude is lower than the true average as a result of the spatial anti-correlation of the spectral sub-types (abridged).

==> ast-2e.tex <==
%%
%% Writing Aids...
%%

\def\etal  {{\em et al.}\relax}
%%
%% From AAS macros...
%%
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\let\la=\lesssim
\let\ga=\gtrsim
\def\ion#1#2{#1$\;${\small\rm\@Roman{#2}}\relax}
%%
%% Journals...
%%\
\def\aj{\ref@jnl{AJ}}
\def\apj{\ref@jnl{ApJ}}
\def\apjl{\ref@jnl{ApJ}}
\def\apjs{\ref@jnl{ApJS}}
\def\apss{\ref@jnl{Ap\&SS}}
\def\aap{\ref@jnl{A\&A}}
\def\aapr{\ref@jnl{A\&A~Rev.}}
\def\aaps{\ref@jnl{A\&AS}}
\def\zap{\ref@jnl{ZAp}}
\def\aplett{\ref@jnl{Astrophys.~Lett.}}
\def\apspr{\ref@jnl{Astrophys.~Space~Phys.~Res.}}
%%
%% Various combinations of units
%%
\def\kms {\hbox{km\,s$^{-1}$}}
\def\AU {{\footnotesize AU}}
\def\solmass {\hbox{\ensuremath{M_\odot}}}
\def\msun {M$_\odot$}
\def\solum {\hbox{\ensuremath{L_\odot}}}
\def\lsun {\solum}
\def\mic {$\mu\hbox{m}$}
%
\def\arcsec {\hbox{$^{\prime\prime}$}}
\def\arcmin {\hbox{$^{\prime}$}}
\def\degree {\hbox{$^{\circ}$}}
\def\hhour {$^{\rm h}$}
\def\mmin {$^{\rm m}$}
\def\ssec {$^{\rm s}$}
\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}
\def\farcm{\hbox{$.\!\!^{\prime}$}}
\def\fdegree {\hbox{$.\!\!^{\circ}$}}
%
\def\cmsq  {\hbox{$\mathrm{cm}^{-2}$}}    %cm-2
\def\percm2  {\hbox{$\mathrm{cm}^{-2}$}}    %cm-2
\def\ccpers {\hbox{${\rm cm}^3{\rm s}^{-1}$}}
\def\percc {\hbox{$\mathrm{cm}^{-3}$}}    %cm-3
\def\CMONE {$\hbox{{\rm cm}}^{-1}$}    %cm-1
\def\cmsix  {$\hbox{{\rm cm}}^{-6}$}  %cm-6
\def\rhounit {$\hbox{M}_\odot\ts \hbox{pc}^{-3}$}
\def\Kkms {\hbox{K\,km\,s$^{-1}$}}
\def\nodat {{ }}

\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}

%%
%%  For Spectroscopy...
%%
\def\n1{N$\;${\small\rm I}\relax}
\def\o1{O$\;${\small\rm I}\relax}
\def\mg2{Mg$\;${\small\rm II}\relax}
\def\si2{Si$\;${\small\rm II}\relax}
\def\s2{S$\;${\small\rm II}\relax}
\def\mn2{Mn$\;${\small\rm II}\relax}
\def\fe2{Fe$\;${\small\rm II}\relax}
\def\zn2{Zn$\;${\small\rm II}\relax}
%
\def\HI{H$\;${\small\rm I}\relax}
\def\HII{H$\;${\small\rm II}\relax}
\def\H2{H$_2$\relax}
\def\Ha{H$\alpha$\relax}
\def\halpha{H$\alpha$\relax}
\def\Hb{H$\beta$\relax}
\def\hbeta{H$\beta$\relax}
\def\oiii{[O$\;${\small\rm III}]\relax}
\def\sii{[S$\;${\small\rm II}]\relax}
\def\nii{[N$\;${\small\rm II}]\relax}

%%
%% Various quantities
%%
\def\Nh{$N_H$\relax}
\def\Nhii  {\hbox{N(H$\;${\small\rm\@Roman{2}}}\relax}
\def\vlsr  {\ensuremath{v_\mathrm{LSR}}}
\def\DH    {\hbox{\ensuremath{n_(\mathrm{H})}}\relax} % n(H)
\def\DMH   {\hbox{${\rm n(H}_{2}{\rm )}$}\relax}      % n(H2)
\def\err   {$\pm$}   % Plus-minus
\def\vsq   {$v^2$\relax}
\def\fwhm  {FWHM\relax}
\def\NTOT  {\ensuremath{N_\mathit{tot}}}
\def\dmh   {\ensuremath{n(\mathrm{H}_2)}}
\def\lgdmh {\ensuremath{\log{[n(\mathrm{H}_2)]}}}
\def\lgdmh {\ensuremath{\log{[n(\mathrm{H}_2)]}}}
\def\logdmh{\lgdmh}
\def\pdot  {\phantom{.}}
\def\pone  {\phantom{0}}
\def\ptwo  {\phantom{00}}
\def\pth   {\phantom{000}}
\def\ptherm{\ensuremath{P_\mathit{therm}}}
\def\PTHERM{\ptherm}


%%
%%Absorption line spectroscopy
%%

\def\Na#1#2{$N_a({\rm #1 \;{\small\rm #2}})$} 
\def\wave#1{$\lambda$#1 \AA\relax}
\def\twowave#1{$\lambda \lambda$#1 \AA\AA\relax}
\def\eqwidth{W$_\lambda$\relax}

\def\ghrs{GHRS}
\def\costar{COSTAR}
\def\fpn{FPN}
\def\Nav{$N_a (v)$}



%%
%%Galaxy Stuff
%%
\def\z{$z$}
\def\Av{$A_V$}

\def\wiyn{WIYN}

